Universal Scalar Leptoquark Action for Matching

In this study we present a universal effective action for one-loop matching of all scalar leptoquarks. We use both the Universal One-Loop Effective Action (UOLEA) and covariant diagrams to evaluate the Wilson coefficients directly in the Green basis for up-to dimension-6 operators. On the technical side, we use the newly developed method of evaluating supertraces, to further validate the results stemming from the use of covariant diagrams. As an application, we perform a fully functional matching onto Standard Model Effective Field Theory (SMEFT) of a model with two scalar leptoquark fields: a weak isospin singlet and a doublet. We demonstrate its use by calculating several observables, such as lepton magnetic and electric dipole moments, neutrino masses, proton decay rate, while we comment upon fine tuning issues in this model. Apart from its phenomenological interest, this model generates the majority of dimension-6 operators and provides an EFT benchmark towards future matching automation.

==> LQs_general_interactions.tex <==
	There are six different scalar leptoquark field representations in isospin space, three singlets, two doublets and one triplet. Their gauge quantum numbers are shown in Table \ref{tab:allcharges}.
%%%%%%%%%%%%%%%%%%%5	
	\begin{table}[h]
		\centering
		\begin{tabular}[c]{| c | c  c  c |}
			\hline
			Field/Group & SU(3) & SU(2) & U(1)\\
			\hline\hline
			$ S_{1} $ & $ \phantom{\displaystyle\frac{1}{1}}\bar{3} $ & $ 1 $ &  $ \frac{1}{3} $\\
			$ \tilde{S}_{1} $ & $ \phantom{\displaystyle\frac{1}{1}}\bar{3} $ & $ 1 $ &  $ \frac{4}{3} $\\
			$ \tilde{S}^{\prime}_{1} $ & $ \phantom{\displaystyle\frac{1}{1}} 3 $ & $ 1 $ &  $ \frac{2}{3} $\\
			$ S_{2} $ & $ \phantom{\displaystyle\frac{1}{1}} 3 $ & $ 2 $ &  $ \frac{7}{6} $\\
			$ \tilde{S}_{2} $ & $ \phantom{\displaystyle\frac{1}{1}} 3 $ & $ 2 $ &  $ \frac{1}{6} $\\
			$ S_{3} $ & $ \phantom{\displaystyle\frac{1}{1}}\bar{3} $ & $ 3 $ &  $ \frac{1}{3} $\\
			\hline
		\end{tabular}
		\caption{All possible representations of a leptoquark under the SM gauge group. The hypercharge is defined so that $ Y_{H} = 1/2 $.}
		\label{tab:allcharges}
	\end{table}	
%%%%%%%%%%%%%%%%%%%%	
	What is common among them is the way they couple to SM fields. We can sketch the interactions of all five leptoquarks with fermions and the Higgs respectively, as shown below,
		\begin{align}
			&S\left(\bar{f}\,f\right), &&SSH, &&SSHH, && SSSH\;,
		\end{align}
	where we collectively denote all leptoquarks with $ S $. All but the second intreaction of the above have dimensionless couplings. The internal structure of the interactions is not in our immediate interest in constructing the effective action, however it is essential in practical applications. As for their self-interactions we can have the following structures,
		\begin{align}
			&SSSS &&\text{and} &&SSS\;,
		\end{align}
	with the triple-$ S $ interaction accompanied by a dimensionful coupling. This "universal" way of writing down leptoquark interactions will be the stepping stone for the calculation of the effective action since these will determine the dimensionality of the $ U $ matrices that we will introduce shortly. 

==> cov_diagrams/orderU2P11.tex <==
\begin{fmffile}{OU2P11}
	\begin{fmfgraph*}(10,10)
		\fmfset{dash_len}{2mm}
		\fmfcurved
		\fmfsurroundn{v}{8}
		\fmfv{d.shape=circle, d.filled=empty,d.size=5}{v3,v5,v7}
		\fmfv{d.shape=circle, d.filled=full,d.size=5,label=$ S $,label.side=right,label.dist=2mm}{v6}
		\fmf{plain,right=.5}{v7,v3}
		\fmf{dbl_dashes,right=1,label=$ S_j $,label.side=right,label.dist=2mm}{v3,v5}
		\fmf{dbl_dashes,right=1,label=$ S_i $,label.side=right,label.dist=2mm}{v5,v7}
		\fmf{dots,width=2,right=.6}{v1,v6}
	\end{fmfgraph*}
\end{fmffile}

==> cov_diagrams/orderU2P12.tex <==
\begin{fmffile}{OU3P12}
	\begin{fmfgraph*}(10,10)
		\fmfset{dash_len}{2mm}
		\fmfcurved
		\fmfsurroundn{v}{8}
		\fmfv{d.shape=circle, d.filled=empty,d.size=5}{v3,v5,v7}
		\fmfv{d.shape=circle, d.filled=full,d.size=5}{v6}
		\fmf{plain,right=1,label=$ f $,label.side=right,label.dist=2mm}{v7,v3}
		\fmf{dbl_dashes,right=.5,label=$ S_j $,label.side=right,label.dist=2mm}{v3,v5}
		\fmf{dbl_dashes,right=.5,label=$ S_i $,label.side=right,label.dist=2mm}{v5,v7}
		\fmf{dots,width=2,right=.3}{v1,v6}
	\end{fmfgraph*}
\end{fmffile}

==> cov_diagrams/orderU2P3_1.tex <==
\begin{fmffile}{OU2P31}
	\begin{fmfgraph*}(10,10)
		\fmfset{dash_len}{2mm}
		\fmfcurved
		\fmfsurroundn{v}{8}
		\fmfv{d.shape=circle, d.filled=empty,d.size=5}{v1,v5}
		\fmfv{d.shape=circle, d.filled=full,d.size=5}{v6,v7,v8}
		\fmf{plain,right=.5,label=$ f $,label.side=right,label.dist=2mm}{v1,v7}
		\fmf{dbl_dashes,right=.4,label=$ S_i $,label.side=right,label.dist=2mm}{v7,v1}
%		\fmf{dots,width=2,right=.5}{v13,v10}
%		\fmf{dots,width=2,right=.5}{v3,v16}
	\end{fmfgraph*}
\end{fmffile}

==> cov_diagrams/orderU2Str.tex <==
\begin{fmffile}{SOU3}
	\begin{fmfgraph*}(10,10)
		\fmfset{dash_len}{2mm}
		\fmfcurved
		\fmfsurroundn{v}{8}
		\fmfv{d.shape=circle, d.filled=empty,d.size=5}{v1,v7,v5}
		\fmf{plain,right=1,label=$ f $,label.side=right,label.dist=1.5mm}{v1,v5}
		\fmf{dbl_dashes,left=0.5,label=$ S_i $,label.side=left,label.dist=1.5mm}{v7,v5}
		\fmf{plain,right=0.5,label=$ f^\prime $,label.side=right,label.dist=.5mm}{v7,v1}
	\end{fmfgraph*}
\end{fmffile}
